Developability Approximation for Neural Implicits through Rank Minimization

Developability refers to the process of creating a surface without any tearing or shearing from a two-dimensional plane. It finds practical applications in the fabrication industry. An essential characteristic of a developable 3D surface is its zero Gaussian curvature, which means that either one or both of the principal curvatures are zero. This paper introduces a method for reconstructing an approximate developable surface from a neural implicit surface. The central idea of our method involves incorporating a regularization term that operates on the second-order derivatives of the neural implicits, effectively promoting zero Gaussian curvature. Implicit surfaces offer the advantage of smoother deformation with infinite resolution, overcoming the high polygonal constraints of state-of-the-art methods using discrete representations. We draw inspiration from the properties of surface curvature and employ rank minimization techniques derived from compressed sensing. Experimental results on both developable and non-developable surfaces, including those affected by noise, validate the generalizability of our method.

==> sec/10_to_write_about.tex <==
1. subgradient method
2. why l1 norm not differentiable - subgradient method pytorch??
3. why nuclear norm minimization vs direct determinant reduction?
4. derivative of determinant of singular matrix 

triangle mesh - cannot processing high tesselation. So have to do mesh simplification to obtain results. the dog has been simplified to 5k vertices. Whereas we do not have such issues


5. influence of marching cubes sampling in train mode.
- if i sample 60k points, then dropout variance results in preventing overfitting 
- but if i sample 250k points, then dropout variance is too low resulting in underfitting
- this the implicit loss is much influenced not by the sdf by rather by first clearning out the overfit, then starting to evaluate.

6. When i use sampling just in eval model, then model ws already overfit that it gets hard to rewire unless we adopt more drop out?



SGP Reviews:
Summary: This paper introduces a neural method for reconstructing piecewise developable or near-developable surfaces from oriented point clouds. The authors leverage the computation of Gaussian curvatures using the Hessian matrix H and propose a developability term that minimizes the rank of H.

The evaluation of the method was conducted on a subset of the ABC dataset, consisting of 1000 CAD models. Additionally, the robustness of the method was tested by introducing noise ranging from 0.5% to 2% level.

Explanation of Recommendation: While the idea of using a developability term is logical for reconstructing surfaces in CAD-like models that are piecewise developable or near-developable, my main concern is the method's practicality due to its dependency on point normals. In the case of noisy models, it remains unclear how the normals for the noisy points were obtained. If the method still requires accurate normals for the noisy points, its usability in real-world scenarios becomes very limited.

Another concern raised is the sensitivity of the method to point distribution. The figures presented in the paper indicate dense and uniformly distributed point clouds. It is important to explore whether the developability term can effectively handle scenarios with sparse and/or non-uniformly distributed points.



-------------------- Review 2 --------------------

Technical Soundness: The following likely has no bearing on the method, but it is a mistake nonetheless: I doubt the NP hardness of the problem stated by (3) What is the size of the input here (against which runtimes are measured)?  It cannot be the size of the input matrix (which is 3x3 always), so the reference to [Nat95] seems not approriate. The relevant complexity is that of simultaneous minimization of a great number of small constant-sized L0 minimization problems which are interdependent in a certain sparse manner. This complexity likely is only polynomial. -- only 7 possible

The relaxations which are used in the paper can still be perfectly useful, of course.  It is only the reference to NP hardness which I feel is a mistake.

Clarity of Exposition: The exposition is reasonably clear


Reproducibility: -


Quality of References: The relevant papers are cited.

The bibliography is rather sloppily done. I looks almost as if the authors had used bibtex records from an unreliable source like Google scholar, instead of actually lookup up their citations. Page numbers and article numbers are often missing. There are even some glaring mistakes like [Tow] or the author list in VNW*20, and some less obvious mistakes like the page numbers in JHR*15. There are typos like pca instead of PCA (I am listing only those I can see at first glance)


Explanation of Recommendation: I am hesitant to recommend publishing this work in its present form.  The reason is that the claim of the paper has not been sufficiently validated. The examples do not show general developable surfaces, only (parts of) planes,  rotational cylinders, rotational cones. Such surfaces have common geometric properties, namely their rotational and translational symmetries, apart from their developability.  The reconstruction of developables in general has not been demonstrated by the paper (BTW for the special surfaces used in the paper, there is prior work on their reconstruction, which works on geometric properties directly and does not need neural networks).


-------------------- Review 4 --------------------

Overall Recommendation: 4 (4 - dubious - not quite acceptable)
Evaluation Confidence: 4 (4 - Pretty confident, I know this area well)

Summary: This paper presents a new loss term for regularizing a DeepSDF-style neural field reconstruction of a 3D shape from a point cloud. The loss term is based on a prior that the underlying surface is developable and hence zero Gaussian curvature almost everywhere. The paper experiments with a few variants of rank minimization on the Hessian of the field. These are all well motivated.


Explanation of Recommendation: Unfortunately, I recommend rejecting this paper from SGP. It bums me out because I read the text before looking at the results and my expectations were that I'd see reconstructions of surfaces that looked obviously close to developability. This is not the case. The results are not much better looking than DeepSDF or PR in this regard. While the curvature metrics are arguing that the they are achieving this to a slight degree, I don't think these experiments are showing that this method is successful. I would really like to see this method succeed and if I were working on it, I'd try some examples where there's no noise and I get a very developable output. I would not worry about generalization over datasets because barely any neural field methods actually do this well.




-------------------- Review 5 --------------------

Overall Recommendation: 5 (5 - marginal - only just acceptable)
Evaluation Confidence: 4 (4 - Pretty confident, I know this area well)

Summary: This paper introduces an optimization of a neural field with a developability-promoting loss. The essence of the loss is to promote the implicit Hessian function to be rank-deficient, and use this loss for reconstruction and fitting. The paper makes the case where such a loss might improve results on the reconstruction of (more or less) developable surfaces, being a prior.

This paper constitutes an interesting attempt at an important problem since many real-life objects are developable or near-developable (because of fabrication constraints). Nevertheless, the evaluation is somewhat underwhelming both in terms of results and in terms of ablations.



a) The role of the latent variable z is not communicated enough (if one is not familiar with deepSDF). What is the purpose of this (and the test-time optimization) that cannot be achieved with a more direct neural-field optimization?

b) In rank minimization, NP-hardness is given as a reason to avoid a loss. However, this is not usually an issue for deep learning that tackles highly non-linear and difficult losses in practice. It is more interesting if a loss is given in variables that allow for effective training with good gradients and usage of data.

c) I'm surprised that minimizing rank(H) (the ambient Hessian) is a good choice rather than minimizing rank(hat(H)) (the implicit Hessian). The Hessian of f(x,y,z) = sqrt(x^2+y^2+z^2) = r has rank two (it's linear in the direction of r. However the level set is a circle which can have any curvature and is certainly not developable.

d) In accordance with point (c), It is not clear if when minimizing for a minimum value on the Hessian, one can discard the denominator |grad(f)|^4. Unless the function is perfectly an SDF, this can have a great impact on the curvature, even if H is very close to minimal rank.

e) I am not sure what to understand from the metric of "how much area has K < delta". Is this a good measure of developability? a surface can have a high-frequency low-amplitude noise which will make it far from developable and still win this metric.

f) It is also not clear what the measure "K" signifies. Moreover, the authors state that they measure both analytic curvature (pointwise) and discrete angle defect (integrated; do you account for dividing by area?). These measures can have very different results between them, which is strongly mesh-related. Which do you use? Is the mesh normalized somehow so that the value of K is relative to anything? Without knowing this it's hard to read Figure 6, where extreme (maybe) values of K=100 appearing red can mask a lot of K between 0 and 100, appearing green.

g) The effects of marching cubes (mostly in terms of resolution) are not discussed; they could be quite major for a sensitive measure like Gaussian curvature, even if the underlying continuous neural field is more or less developable.





==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/6_results.tex <==
\section{result}
\paragraph*{observation}

determinant minimization gives piecewise planar developable reconstruction
logdet gives smooth developable surface reconstruction
svd3 gives
l1 norm gives

